Scalable Multi-Hop Relational Reasoning for Knowledge-Aware Question Answering

Existing work on augmenting question answering (QA) models with external knowledge (e.g., knowledge graphs) either struggle to model multi-hop relations efficiently, or lack transparency into the model's prediction rationale. In this paper, we propose a novel knowledge-aware approach that equips pre-trained language models (PTLMs) with a multi-hop relational reasoning module, named multi-hop graph relation network (MHGRN). It performs multi-hop, multi-relational reasoning over subgraphs extracted from external knowledge graphs. The proposed reasoning module unifies path-based reasoning methods and graph neural networks to achieve better interpretability and scalability. We also empirically show its effectiveness and scalability on CommonsenseQA and OpenbookQA datasets, and interpret its behaviors with case studies.

==> intro-old.tex <==

% %%% 1st paragraph: . 1. what is NLI and its importance; 2. how existing deep neural models (e.g., the pre-train models) work on this task and what are their limitations; 3. Transit to the needs of structured knowledge, and conclude that we need to find ways to augmented such models with external, structured knowledge like those in knowledge graphs.
% One of the great challenges of intelligence is to understand the nature of cognition so well that machines can be made to exhibit human-like reasoning abilities \citep{Harmelen2008HandbookOK}. Statistical learning is being well explored as a most popular AI approach. Such learning takes the analogy from human's pattern recognition and falls into the paradigm of connectionism in continuous space. In this setting, a model is to best fit the observed data and recognize unobserved ones given the assumption of independent and identically distributions. On the other hand, symbolicism regards discrete logic as the core of intelligence, which strikes a chord with Universal Grammar's postulation: a certain set of \textit{structural} rules are innate to humans, independent of sensory experience. Intelligence could thus be formalized as symbolic reasoning with explicit representations of knowledge. This paradigm, owing to the nature of reasoning, has the potential to understand and generate unseen representations and knowledge, performing reason-based categorization.
% \xiang{I think we don't need to go this broad to start. For the first paragraph, probably we can go as: 1. what is NLI and its importance; 2. how existing deep neural models (e.g., the pre-train models) work on this task and what are their limitations; 3. conclude that we need to find ways to augmented such models with external, structured knowledge like those in knowledge graphs.}
% %neural-symbolic integration?

% Despite extensive success of large-scale pretrained language models, gap still exists between human intelligence and such statistical neural models. In the field of natural language understanding, analysis \citep{petroni2019language} show that although these models can capture and store relational knowledge in textual corpora, partially functioning as a latent knowledge base, they still predict relations between objects largely based on co-occurrence instead of logical reasoning. 
% \xiang{can merge to the 1st paragraph per above comments.}

% %%% 2nd paragraph: 1. Summary of prior work on augmenting models with external structured knowledge. 2. Transit to discuss the line of work modeling the related structured knowledge and their limitations.
% On the other hand, empowering neural models with knowledge graphs as sources of external information is deemed beneficial for models' performance and explainability in recent NLU tasks. Entity embeddings as a basic unit for knowledge injection into neural models might be a most straightforward approach~\citep{Yang2017LeveragingKB, Zhang2019ERNIEEL}. Alternatively, there are attempts to encode facts in the form of triples or text-form triples as basic knowledge blocks~\citep{weissenborn2017dynamic, Mihaylov2018KnowledgeableRE}. The key intuition of such work is to attentively retrieve facts from external sources to mitigate the absence of required world knowledge. In this case, external knowledge utilization comes in the form of information retrieval and integration with text. These models have access to local properties and latent relations but hardly can they explicitly form logical chains and account for the predictions. 

% Explicitly modeling relational subgraphs of KGs to aid language understanding is closer to neural-symbolic integration.  \citet{kagnet-emnlp19,bauerwang2019commonsense} treat relational paths, graphs with constraints, as natural reasoning units. However, the path-level nature limits scalability in terms of path length and extraction of such constrained sub-graphs is naturally non-differentiable. Another direction focuses on general graph encoding using graph neural networks. But there is no in-place graph architecture specialized in explicit reasoning in this domain.
% \xiang{Merge into the prior paragraph. The flow of 2nd paragraph: 1. Summary of prior work on augmenting models with external structured knowledge. 2. Transit to discuss the line of work modeling the related structured knowledge and their limitations.}


% %%% 3rd paragraph: our solution ideas and technical contributions
% % - higher-order relation within layer
% % - scalability of gnn
% % - semantic guidance
% % typed nodes > relation network
% In this work, we introduce \textit{Multi-hop Relational Graph Network}, an extension of graph neural network designed for semantics-aware relational reasoning. Our proposed network is applicable to graphs with heterogeneous nodes and relational edges. Nodes in this network are \textit{typed} according to their properties in different natural language understanding tasks. \xiang{a bit hard to follow here as the ``types" here are unclear.} Within a single layer of message passing, our model encodes the neighboring $K$-hop relational paths in a node-type-specific way to prepare for state updates. From this perspective, our work is associated with Relation Networks (RNs)~\citep{Santoro2017ASN} in that we represent higher-order relational information between symbolic nodes as the aggregation of multi-hop paths. \xiang{can we connect to aforementioned limitations and stress more on why this idea can help?} Moreover, our model is scalable in terms of the number of node types without potential combinatorial computations in the original paradigm of RNs. In the meantime, our model enjoys the scalability of general neural networks compared with aforementioned path-based models and is free to explore beyond the limitations of path-structured constraints. \xiang{maybe just directly say that a straightforward implementation of the idea will be intractable becuase of xxx, and we do xxx to make it scalable?} Drawing inspirations from conditional random fields \citep{Lafferty2001ConditionalRF},  we further design text-centric high-order attention mechanism upon relational paths, providing semantic guidance in a much more fine-grained manner.  This part is also in line with our intention of integrating symbolic reasoning into neural models. \xiang{what aforementioned limitation/issue does this idea tackle? say it out.}
% \xiang{highlight }

% \xiang{4th part: Add a summary of maybe 3 contribution bullets, including one on experiment findings and positive results.}

% % Graph neural networks have brought excitement in many natural language processing tasks. (\cite{DBLP:journals/corr/abs-1809-10185}) However, their applications in this domain are generally restricted to either node-level or graph-level point of view as a means of information propagation inside graphs. On the other hand, the potential of graph neural networks for logical reasoning is rarely exploited.

% % Empowering neural models with knowledge graphs as sources of external information is deemed useful in recent NLI tasks. \cite{DBLP:journals/corr/abs-1805-07858} inject external knowledge by either attending to fact triples in KGs or enriching text representations with node embeddings pretrained on KGs, in which case the model has access to local properties and latent relations but hardly can it explicitly examine logical chains to account for models' predictions. Following this line are work that explicitly model relational subgraphs of KGs to aid language understanding. \cite{kagnet-emnlp19} approach knowledge-aware question answering in a path-level point of view, encoding paths between key concepts in questions and answers using RNNs. Nevertheless, path-level learning can hardly scale to maximum length of paths. And the process of path extraction is non-differentiable.

% % \begin{enumerate}
% %     \item Current multi-hop GNNs cannot handle relational graphs
% %     \item Our model can perform logical reasoning upon relational graph while matching the semantics of context, providing knowledge and evidence for natural language understanding.
% % \end{enumerate}

==> intro_v1.tex <==
\section{Introduction}
\label{sec:intro}
Recently, there have been Question Answering (QA) datasets~\citep{Talmor2018CommonsenseQAAQ, Sap2019SocialIQACR, clark2018think,Mihaylov2018CanAS} that require not only \textit{textual} understanding, but also \textit{relational reasoning} over the entities in text. For example, the question in Fig.~\ref{fig:example} requires models to perform relational reasoning over mentioned entities, $\ie$, to infer latent relations between $\{$\textsc{Child}, \textsc{Sit}, \textsc{Desk}, \textsc{Schoolroom}$\}$. Facts such as \textit{a child is likely to appear in a schoolroom} may not be readily contained in the question itself, but commonsensical to human through learning and experiences. Therefore, many~\citep{Mihaylov2018KnowledgeableRE,kagnet-emnlp19,Wang2018ImprovingNL,yang-etal-2019-enhancing-pre} turn to structured knowledge graphs, which distils relational knowledge between entities into multi-relational edges, for models' knowledge acquisition and relational reasoning.

\input{figures/example.tex}

Despite the success of large-scale pre-trained language models (LMs)~\cite{Devlin2019BERTPO,Liu2019RoBERTaAR}, there is still a large performance gap between these models and human performance on datasets that probe relational reasoning. They also fall short of providing interpretable predictions because knowledge in their pre-training corpus resides in a latent way, making it hard to recover the reasoning process. Incorporating knowledge graphs, however, brings the potential of interpretable and trustworthy predictions. For example, in Fig.~\ref{fig:example}, the relational path $(\textsc{Child}\rightarrow \texttt{AtLocation}\rightarrow \textsc{Classroom}\rightarrow \texttt{Synonym}\rightarrow \textsc{Schoolroom})$ naturally provides evidence for the answer \textsc{Schoolroom}. 

% Reasoning over structured relational data is not self-evident. In a knowledge graph, relations between entities are \textit{structured}, manifested as the compositional aggregation of entities and relational edges that interconnect them.
A straightforward approach to leveraging knowledge graph is thus to directly model these relational paths. KagNet~\citep{kagnet-emnlp19} and MHPGM~\citep{bauer-etal-2018-commonsense} extract relational paths from knowledge graph and encode them with sequence models, in which case high-order relations are explicitly modeled. Application of attention mechanisms upon these relational paths can further offer good interpretability. However, these models are hardly scalable because the number of possible paths in a graph is  (1)  polynomial w.r.t. the number of nodes (2) exponential w.r.t. the path length (see Fig.~\ref{fig:scalability}). Therefore, some~\citep{weissenborn2017dynamic, Mihaylov2018KnowledgeableRE} resort to only using one-hop paths, namely, triples, to balance scalability and reasoning capacities.

Alternatively, Relational GCN~\citep{Schlichtkrull2017ModelingRD} perform message passing between neighboring nodes with relation type as an additional modifier,

Alternatively, Graph Neural Networks (GNNs) are designed to work directly on graph structures. Each node exchanges information with its neighboring nodes until an equilibrium is reached. Graph Convolutional Networks (GCNs)~\citep{Kipf2016SemiSupervisedCW} are variants of GNNs, where transformation matrices for message passing from neighbors are shared among all nodes. However, they can't model relational graphs as edge types are not taken into consideration. Relational Graph Convolutional Networks (RGCNs)~\citep{Schlichtkrull2017ModelingRD} use different transformation matrices for message passing on edges of different relational types, thus are capable of encoding multi-relational graphs. The message passing process for GNNs can be efficiently implemented as matrix multiplication, leading to good scalability. However, because messages are passed from direct neighbors and features are aggregated at node level, multi-hop logical paths, which are vital to reasoning, can hardly be interpreted from GNNs.

% Alternatively, Relational GCN~\citep{Schlichtkrull2017ModelingRD} perform message passing between neighboring nodes with relation type as an additional modifier, in which case multi-hop information flows are implicitly mingled and buried across layers. 
% The complementary advantages of RGCN and path-based models motivate us to empower graph networks with explicit multi-hop relational reasoning.



% Despite the success of large-scale pre-trained language models (LMs)~\cite{Devlin2019BERTPO,Liu2019RoBERTaAR}, there is still a large performance gap between these models and human performance. This may be attributed to two reasons: 1) the textual knowledge from pre-training corpora is insufficient 2) they do not fully \textit{comprehend} latent knowledge~\citep{petroni2019language}.
%Although self-attention mechanism helps justify the prediction, the concrete reasoning process over knowledge to arrive at the prediction remains unclear.


% 1. we enhance the performance of models by performing relational reasoning over structured knowledge

% RR is the method to incorporate KG

% 2.we enhance the relational reasoning ability of models by incorporating structured knowledge
% RR is the purpose of incorporate KG




\input{figures/scalability.tex}

% One of the great challenges of intelligence is to reason about entities and their properties, namely, perform \textit{relational reasoning} over discrete entities. The aforementioned tasks also probe relational reasoning over entities in text with external knowledge as inductive bias. This ability is also critical to interpretable and trustworthy predictions. On the other hand, the nature of \textit{structured} knowledge graph brings about the potential of both reasoning and interpretability. Some~\citep{Yang2017LeveragingKB, Zhang2019ERNIEEL} seek to exploit the complementary strengths of neural models and \textit{structured} knowledge and use entity embeddings as a basic unit for knowledge injection into neural models. In this case, the relations between entities are implicit in distributional representations, which hinders their reasoning capacity.

% Relational reasoning over structured relational data is not self-evident. In a knowledge graph, relations between entities are \textit{structured}, manifested as the compositional aggregation of entities and relational edges that interconnect them. Relational GCN~\citep{Schlichtkrull2017ModelingRD} perform message passing between neighboring nodes with relation type as an additional modifier, in which case multi-hop information flows are implicitly mingled and buried across layers. Alternatively, path-based approaches ~\citep{kagnet-emnlp19,bauer-etal-2018-commonsense} explicitly extract relational paths from knowledge graph and encode them to form multi-hop reasoning units. But the path-level nature limits scalability with respect to path length. Therefore, some~\citep{weissenborn2017dynamic, Mihaylov2018KnowledgeableRE} resort to only using one-hop paths, namely, triples, to balance scalability and knowledge integration, at the cost of multi-hop reasoning abilities. The complementary advantages of RGCN and path-based models motivate us to empower graph networks with explicit multi-hop relational reasoning.


% One of the great challenges of intelligence is to reason about entities and their properties, namely, perform \textit{relational  reasoning} over discrete entities. While large-scale pre-trained language models have achieved extensive success across various NLP tasks, recent analysis \citep{petroni2019language} shows that although these models can capture and store relational knowledge, partially functioning as latent knowledge bases, they still predict relations between objects largely based on co-occurrence instead of reasoning. Another issue with these models is interpretability. 
% Although self-attention mechanism helps justify the prediction, the concrete reasoning process to arrive at the prediction remains unclear.
% % \xiang{can compress further.}


% Many seek to exploit the complementary strengths of neural models and structured knowledge in NLP tasks that require both textual context understanding and commonsense knowledge~\citep{Talmor2018CommonsenseQAAQ,Mihaylov2018CanAS,Sap2019SocialIQACR}. 
% Entity embeddings as a basic unit for knowledge injection into neural models might be the most straightforward approach~\citep{Yang2017LeveragingKB, Zhang2019ERNIEEL}. 
% In this case, the relations between entities are implicit in distributional representations, which makes it hard for models to explicitly account for their predictions.

In this paper, we propose a novel graph encoding architecture, called \textit{Multi-hop Graph Relation Network} (MultiGRN), which is an extension of graph neural network designed for context-aware relational reasoning. Our proposed network is applicable to graphs with heterogeneous nodes and relational edges. Nodes in the graph are \textit{typed} according to their properties in different natural language understanding tasks.  In question answering tasks, we distinguish between entities whose mentions appear in the question, answer, or neither. Within a single layer of message passing, our model encodes the neighboring $K$-hop relational paths in a node-type-specific way to prepare for state updates. Our work is associated with Relation Networks ~\citep{Santoro2017ASN} in that we represent higher-order relational information between symbolic entities as the aggregation of multi-hop paths. In the meantime, our model enjoys the scalability of general graph neural networks compared with aforementioned path-based models. 
% and is free to explore beyond the limitations of path-structure constraint
Drawing inspirations from conditional random fields \citep{Lafferty2001ConditionalRF}, we further design text-centric structured attention mechanism upon relational paths, providing semantic guidance in a more fine-grained manner. 

\input{tables/model_properties.tex}

We outline the favorable features of knowledge-aware QA models in Table~\ref{tab:property} and compare our MultiGRN with representative GNNs and path-based methods. The main contributions of this work are summarized as follows: 
\begin{itemize}
\item We propose MultiGRN, a novel model architecture tailored to multi-hop relational reasoning. Our model is capable of explicitly modeling multi-hop relational paths while preserving good scalability.
\item We propose structured relational attention mechanism for efficient and interpretable modeling of multi-hop relational paths, along with its training and inference algorithm.
\item We conduct extensive experiments on two question answering datasets and show that our models bring significant improvements compared to knowledge-agnostic pre-trained language models, and outperform other graph encoding methods by a large margin.
\end{itemize}
% \xiang{Add a summary of maybe 3 contribution bullets, including one on experiment findings and positive results.}







% %%% 1st paragraph: . 1. what is NLI and its importance; 2. how existing deep neural models (e.g., the pre-train models) work on this task and what are their limitations; 3. Transit to the needs of structured knowledge, and conclude that we need to find ways to augmented such models with external, structured knowledge like those in knowledge graphs.

% %%% 2nd paragraph: 1. Summary of prior work on augmenting models with external structured knowledge. 2. Transit to discuss the line of work modeling the related structured knowledge and their limitations.

% %%% 3rd paragraph: our solution ideas and technical contributions
% % - higher-order relation within layer
% % - scalability of gnn
% % - semantic guidance
% % typed nodes > relation network

% %%% 4th part: Add a summary of maybe 3 contribution bullets, including one on experiment findings and positive results.



==> tables/compatibility.tex <==
\begin{table}[t]
% \vspace{-0.1cm}
\centering
\scalebox{0.8}{
\begin{tabular}{@{}lcc@{}}
    \toprule
    \textbf{Methods} & Dev-Acc. (\%)  & Test-Acc. (\%) \\
    \midrule
    AristoRoBERTaV7\textsuperscript{\dag} & 79.2 & 77.8 \\
    {~+ MHGRN ($K=3$)} & 78.6 & 80.6 \\
    \bottomrule
\end{tabular}
}
% \vspace{-0.2cm}
\caption{Performance comparison between vanilla AristoRoBERTaV7 and AristoRoBERTaV7+MHGRN.}
\label{tab:results:compatibility}
% \vspace{-0.0cm}
\end{table}

==> tables/evidence.tex <==
\begin{table}[h]
\centering
\scalebox{0.6}{
\begin{tabular}{l|c}
  \toprule
  \textbf{Question} & {Where is known for a multitude of wedding chapels?} \\ 
  \midrule
  \textbf{Options} & {A. town~~~B. Texas~~~C. city~~~D. church buildings~~~E. Nevada} \\
  \textbf{Answer} & {E. Nevada} \\
  \textbf{Path Evidence} & {$\textsc{Chapel}\rightarrow \texttt{AtLocation}\rightarrow \textsc{Reno} \rightarrow \texttt{partof}\rightarrow\textsc{Nevada}$}  \\
  \bottomrule
\end{tabular}
}
\caption{A sample question with the reasoning path output by MultiGRN.}
\label{tab:evidence}
\end{table}
